Randomness Requirements for Three-Secret Sharing

We study a secret sharing problem with three secrets where the secrets are allowed to be related to each other, i.e., only certain combinations of the three secrets are permitted. The dealer produces three shares such that every pair of shares reveals a unique secret and reveals nothing about the other two secrets, other than what can be inferred from the revealed secret. For the case of binary secrets, we exactly determine the minimum amount of randomness required by the dealer, for each possible set of permitted combinations. Our characterization is based on new lower and upper bounds.

==> bigcube.tex <==
\newcommand{\Depths}{2}
\newcommand{\Heights}{2}
\newcommand{\Widths}{2}

\newcommand \drawcubeas[1]
{
    \coordinate (O) at (#1,0,0);
    \coordinate (C) at (#1,\Heights,0);
    \coordinate (G) at (#1,\Heights,\Depths);
    \coordinate (D) at (#1,0,\Depths);
    \coordinate (A) at (\Widths+#1,0,0);
    \coordinate (B) at (\Widths+#1,\Heights,0);
    \coordinate (F) at (\Widths+#1,\Heights,\Depths);
    \coordinate (E) at (\Widths+#1,0,\Depths);
    
    \draw (O) -- (A) -- (E) -- (D) -- cycle;% Bottom Face
    \draw (C) -- (B) -- (F) -- (G) -- cycle;% Top Face
    \draw (O) -- (C);
    \draw (A) -- (B);
    \draw (E) -- (F);
    \draw (D) -- (G);
}

\newcommand \drawballbig[1]
{
    \shade[ ball color = red, opacity = 1.0] (#1) circle (0.2 cm);
}

\begin{figure}
\label{fig:bigcube}

\begin{tikzpicture}
    \drawcubeas{0}
    %% \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
    %\foreach \ballcoord in {{O},{D},{C},{G},{A},{E},{B},{F}}
    %{
    %    \drawballbig{\ballcoord}
    %}
    \node [below] at (O) {$(000)$};
    \node [below] at (A) {$(100)$};
    \node [below] at (E) {$(101)$};
    \node [below] at (D) {$(001)$};
    \node [above] at (C) {$(010)$};
    \node [above] at (B) {$(110)$};
    \node [above] at (F) {$(111)$};
    \node [above] at (G) {$(011)$};
\end{tikzpicture}
\caption{Points in $\{0,1\}^3$: The spheres correspond to the points in a support.}
\end{figure}


==> hari.tex <==
% We study the following multiple secret sharing problem. There are three secrets $\xa,\xb$ and $\xc$ with alphabets $\cXa, \cXb$ and  $\cXc$ respectively intended for three different parties $\pa, \pb$ and  $\pins$ respectively. The secrets are {\em correlated} in the sense that they are known to be from a subset $\cS \subseteq \cXa \times \cXb \times \cXc$. The dealer produces three different shares $\Sab,\Sbc,\Sca$ and distributes it as follows: party $\pa$ receives shares $\Sab,\Sca$; party $\pb$ receives shares $\Sab,\Sbc$; and party $\pins$ receives $\Sbc,\Sca$. The goal of the dealer is to produce these shares such that the parties may recover the secrets intended for them without acquiring any additional information about the other secrets other than what they may infer from their own secret. To accomplish this, the dealer is given access to private randomness $R$ sampled from a space $\cR$ having a distribution $P_R$. Let $\Sa = (\Sab, \Sca)$, $\Sb = (\Sab, \Sbc)$, $\Sc = (\Sca, \Sbc)$ and $\s = (\Sab, \Sbc, \Sca)$. Let the shares $\Sab, \Sbc$ and $\Sca$ be sampled from the share spaces $\salpab, \salpbc$ and $\salpca$ respectively, $\salp = \salpab \times \salpbc \times \salpca$, $\salp_1 = \salpab \times \salpca$, $\salp_2 = \salpbc \times \salpab$ and $\salp_3 = \salpca \times \salpbc$. Also, for ease of notation, let $\cN=\{1,2,3\}$, $\s_{i,j} = \s_{j,i}$ and $\salp_{i,j} = \salp_{j,i}$ for any $i,j \in \cN$. We also denote $\x =(\Xa,\Xb,\Xc)$ and $x = (x_a,x_b,x_c)$.

% \begin{definition}
% A secret sharing scheme $\scheme$ with randomness alphabet $\cR$ having a distribution $P_R$ consists of a encoding function $\encoder : \cS \times \cR \longrightarrow \salp$ and a decoding function $\decoder_i: \salp_i \longrightarrow \cS_i$ at party $i$ where $i \in \cN$.
% \end{definition}
% For $x=(\xa,\xb,\xc) \in \cS$ and $r \in \cR$, $P_{\s|\x,R}(w|x,r) = \mathbb{1}_{\{w=\encoder (x,r)\}}$. The randomness $R$ induces a distribution on the shares $W$ conditional on the secrets in the following manner:
% $$P_{\s|\x}(w|x) = \sum_{r \in \cR} P_{\s,R|\x}(w,r|x) = \sum_{r \in \cR} P_R(r) \mathbb{1}_{\{w=\encoder(x,r)\}} \text{.}$$


% \textbf{Correctness and Privacy Criteria}
% \begin{definition}
% A secret sharing scheme $\scheme$ generating shares according to the distribution $p_{\s|\Xa,\Xb,\Xc}$ is said to be correct if 
% \begin{multline}
% \forall (i,j,k) \leftarrow \cN,\\ \forall (x_i, x_j, x_k), (x_i', x_j', x_k') \in \cS \text{ such that } x_i \neq x_i',\\ \text{ there is no } \siabc \in \salp_i \text{ for which } P_{\s_i|\x}(\siabc|x_i,x_j,x_k)>0 \text{ and } \\ P_{\s_i|\x}(\siabc|x_i',x_j',x_k')>0
%  \end{multline}
% \end{definition}

% This implies that, a secret sharing scheme $\scheme$ generating shares according to the distribution $p_{\s|\Xa, \Xb, \Xc}$ is said to be correct if 
% \begin{align}
% \label{corr1}
% H(\Xa | \Sab, \Sca)=0,\\
% \label{corr2}
% H(\Xb | \Sab, \Sbc)=0,\\
% \label{corr3}
% H(\Xc | \Sca, \Sbc)=0
% \end{align} for any distribution $P_{\Xa,\Xb,\Xc}(\xa,\xb,\xc)$ where $(\xb,\xb,\xc) \in \cS$.

% \begin{definition}
% A secret sharing scheme $\scheme$ generating shares according to the distribution $p_{\s|\Xa,\Xb,\Xc}$ is said to be private if 
% \begin{multline}
%     \forall (i,j,k) \leftarrow \cN\, \\
%     \forall(x_i,x_j,x_k), (x_i,x_j',x_k') \in \cS, \forall \siabc \in \salp_i, \\
%     P_{\s_i|\Xa,\Xb,\Xc}(\siabc|x_i,x_j,x_k) = P_{\s|\Xa,\Xb,\Xc}(\siabc|x_i,x_j',x_k')
% \end{multline}
% \end{definition}
% This implies that the secret sharing scheme $\scheme$ generating shares according to the distribution $p_{\s|\Xa, \Xb, \Xc}$ is said to be private if the following holds:
% \begin{align}
% \label{priv1}
% I(\Sa;\Xc,\Xb|\Xa)=0,\\
% \label{priv2}
% I(\Sb;\Xa,\Xc|\Xb)=0,\\
% \label{priv3}
% I(\Sc;\Xb,\Xa|\Xc)=0
% \end{align} for any distribution $p_{\Xa,\Xb,\Xc}(\xa,\xb,\xc)$ where $(\xa,\xb,\xc) \in \cS$.

% \begin{definition}
% The randomness complexity for a scheme $\scheme$ which generates the shares according to the distribution $P_{\s_i|\Xa,\Xb,\Xc}$ with randomness alphabet $\cR$ is defined as
% \begin{equation}
% \rc = \log |\cR|
% \end{equation}
% \end{definition}

\textbf{Common Information and Residual Information}\\
Let $X$ and $Y$ be two random variable taking values in $\cX$ and $\cY$ jointly distributed as some $p_{XY}$. Consider a random variable $Q$ taking values in $\cQ$ such that $Q=f(X)=g(Y)$ for some functions $f:\cX \longrightarrow \cQ$ and $g:\cY \longrightarrow \cQ$. The G\'acs-K\"orner common information \cite{} is the maximum possible entropy of $Q$. We denote this common information with $CI_{GK}(X;Y)$. The common variable is defined as $Q^*= \arg \max_{f(X)=g(Y)=Q} H(Q)$. The difference between mutual information and common information is the residual information $RI(X;Y)$. 
$$RI(X;Y) = I(X;Y) - CI_{GK}(X;Y)$$
The following definition of residual information from \cite{} is used here.

\begin{definition}
    The residual information of jointly distributed random variables $X,Y$ and $Q$ is given by
    \begin{equation}
    \label{ridef}
        RI(X;Y):= \min_{\substack{p_{Q|X,Y}\\ I(Q;Y|X)=I(Q;X|Y)=0}} I(X;Y|Q)
    \end{equation}
\end{definition}
The minimizing $Q$ here is the common random variable. So, the residual information between $X$ and $Y$ is the mutual information between $X$ and $Y$ conditioned on $Q^*$. 

\begin{definition}
    Consider a probability distribution $P_{X,Y}$ such that $X$ is sampled from $\cX$ and $Y$ is sampled from $\cY$. The characteristic bipartite graph of $P_{X,Y}$ is defined as the graph $G=(V,E)$ such that $V = \cX \times \cY$ and for $x \in \cX, y \in \cY, \exists\+ e(u,v) \in E $ whenever $P_{X,Y}(x,y)>0$. 
\end{definition}
The random variable induced by the connected components of the characteristic bipartite graph of $(X,Y)$ is the equal to the common random variable. 

\begin{lemma}
\cite{} If $T,U,V,Z$ are jointly distributed random variables such that the following two conditions hold: $I(U;Z|T)=0$ and $I(T;V|Z)=0$. Then, 
\begin{equation}
\label{ridpineq}
RI(T;Z) \leq RI((U,T);(V,Z))
\end{equation}
\end{lemma}

\begin{lemma}
    \label{naivelemma}
    For a scheme $\scheme$ generating shares according to the distribution $P_{\Shares|\Secrets}$, the following holds
    \begin{align}
    \label{naivelemma1}
    H(\Sbc|\Sab, \Sca) \geq H(\Xb,\Xc|\Xa)\\
    \label{naivelemma2}
    H(\Sca|\Sab, \Sbc) \geq H(\Xc,\Xa|\Xb)\\
    \label{naivelemma3}
     H(\Sab|\Sca, \Sbc) \geq H(\Xa,\Xb|\Xc)
    \end{align}

    \begin{proof}
    We will prove this for (\ref{naivelemma1}) and (\ref{naivelemma2}) and (\ref{naivelemma3}) follow from symmetry on the parties. 
    \begin{align*}
    H(\Sbc|\Sab, \Sca) &\stackrel{(a)}{=} H(\Xa, \Sbc|\Sab, \Sca)\\
    & \stackrel{(b)}{\geq} H(\Sbc| \Sab, \Sca, \Xa)\\
    & \stackrel{(c)}{=} H(\Xb, \Xc, \Sbc|\Sab, \Sca, \Xa)\\
    & \stackrel{(d)}{\geq} H(\Xb, \Xc|\Sab, \Sca, \Xa)\\
    & \stackrel{(e)}{=} H(\Xb, \Xc|\Xa)
    \end{align*}
    where (a) follows from the correctness criteria (\ref{corr1}), (c) follows from correctness criteria (\ref{corr2}) and (\ref{corr3}), (b) and (d) follow from chain rule of entropy and (e) follows from the privacy criteria (\ref{priv1}).
    \end{proof}
    This lemma states that the uncertainty in the share on the opposite edge will be at least as much as the uncertainty in the other secrets. This is due to the fact that shares may be of arbitrarily large size. 
\end{lemma}

\begin{lemma}
    \label{rilemma}
    For a secret sharing scheme $\scheme$ generating shares according to $P_{\Shares|\Secrets}$, the following relations hold
    \begin{align}
    \label{rilemma1} 
    I(\Sab;\Sbc|\Sca) \geq RI(\Xa;\Xc)\\
    \label{rilemma2}
    I(\Sbc;\Sca|\Sab) \geq RI(\Xa;\Xb)\\
    \label{rilemma3}
    I(\Sca;\Sab|\Sbc) \geq RI(\Xb;\Xc)
    \end{align}
\end{lemma}
\begin{proof}
    We prove this lemma for (\ref{rilemma1}) and the argument for (\ref{rilemma2}) and (\ref{rilemma3}) follow from symmetry on the parties.
    \begin{align*}
        I(\Sab;\Sbc|\Sca) &= I(\Sab,\Sca;\Sbc,\Sca|\Sca)\\
        & \stackrel{(a)}{=} I(\Sab,\Sca,\Xa; \Sbc,\Sca,\Xc|\Sca)\\
        & = I(\Sa,\Xa;\Sc,\Xc|\Sca)
    \end{align*}
    Since $I(\Sca;\Xc,\Sc|\Xa,\Sa) = I(\Sca;\Xa,\Sa|\Xc,\Sc) = 0$, 
    \begin{align}
        I(\Sa,\Xa;\Sc,\Xc|\Sca) &\stackrel{(b)}{\geq} RI(\Sa,\Xa;\Sc,\Xc)\\
        &\stackrel{(c)}{\geq} RI(\Xa;\Xc)
    \end{align}
    where (a) follows from correctness conditions (\ref{corr1}) and (\ref{corr3}) and (b) follows from the definition of residual information (\ref{ridef}). (c) follows from the secure data processing inequality (\ref{ridpineq}) where $I(\Xa;\Sa|\Xc)=I(\Xc;\Sc|\Xa)=0$ comes from privacy conditions.
\end{proof}

% \section{Developing the Lower Bound}
% We will develop the lower bound through an optimization process done in a certain fashion. With the help of lemma \ref{viewlemma} and corollary \ref{viewcorollary}, we develop a bound on the randomness complexity in terms of entropy of the shares and the secrets.
% \begin{lemma}
% \label{viewlemma}
%     For a scheme $\scheme$ generating shares according to the distribution $P_{\s|\x}$ and $\x$ being distributed according to $P_{\X}$,
%     \begin{equation}
%         H(\s|\x) \geq \max_{i}\{H(\s_{i}) - H(\x_i)\}
%     \end{equation}
% \end{lemma}
% \begin{proof}
%     \begin{align*}
%         H(\s|\x) &= H(\Sab,\Sbc,\Sca|\Xa,\Xb,\Xc)\\
%         &\stackrel{(a)}{\geq} \max\{H(\s_1|\x), H(\s_2|\x), H(\s_3|\x)\}\\
%         & \stackrel{(b)}{\geq} \max\{H(\s_1|\\xa), H(\s_2|\\xb), H(\s_3|\\xc)\}\\
%         & = \max_{i}\{H(\s_i|\x_i)\}\\
%         & \stackrel{(c)}{\geq} \max_{i}\{H(\s_i) - H(\x_i)\}
%     \end{align*}
%     where (a) and (c) are because of chain rule and (b) is because of privacy conditions (\ref{priv1}), (\ref{priv2}) and (\ref{priv3}).
% \end{proof}


% \begin{corollary}
% \label{viewcorollary}
%     For a secret sharing scheme $\Pi$ generating shares according to the distribution $P_{W|X}$ and $X$ sampled from the space $\cS$,
%     \begin{align}
%         \rc &\geq \max_{P_{\X} \in \cP_{\cS}} H(\s|\x)\\ &= \max_{P_{\X} \in \cP_{\cS}} \max_{i}\{H(\s_i) - H(\x_i)\}\\ &= \max_{i} \max_{P_{\X} \in \cP_{\cS}} \{H(\s_i) - H(\x_i)\}
%     \end{align}
% \end{corollary}

% For any $i \in \cN$, $H(\s_i) = H(\s_{i,j},\s_{j,k})$ such that $j,k \in \cN$ and $i \neq j \neq k$. This is equivalent to $H(\s_i) = H(\s_{i,j}, \s_{i,k})$ where $(i,j,k)$ is a permutation on $\cN$. The corollary can be re-written as
% \begin{equation}
% \rc \geq \max_{(i,j,k)\leftarrow \cN} \max_{P_{\X} \in \cP_{\cS}} \{H(\s_{i,j},\s_{i,k}) - H(\x_i)\}
% \end{equation}

% \begin{lemma}
% \label{lemmab1b2}
%     For a given scheme $\scheme$ which generates shares according to the distribution $P_{W|X}$ such that $X$ is coming from a space $\cS$ and any permutation $(i,j,k)$ of $\cN$,
%     \begin{multline}
%         \max_{P_{\X} \in \cP_{\cS}} \{H(\s_i)-H(\x_i) \} \geq \max_{P_{\X}\in \cP_{\cS}}\{B_1^{(i,j,k)},B_2^{(i,j,k)}\} \\= \max\left\{\max_{P_{\X} \in \cP_{\cS}} B_1^{(i,j,k)}, \max_{P_{\X} \in \cP_{\cS}} B_2^{(i,j,k)}\right\}
%     \end{multline}
%     where $B_1^{(i,j,k)} = H(\s_{i,j}|\s_{k,i}) + H(\s_{k,i}|\s_{i,j}) - H(\x_i)$ and $B_2^{(i,j,k)} = H(\s_{i,j}|\s_{j,k}) + H(\s_{k,i}|\s_{i,j}) - H(\x_i)$.
% \end{lemma}
% \begin{proof}
% Expanding further, we have 
% \begin{equation}
%     H(\s_{i,j},\s_{i,k}) = H(\s_{i,j}) + H(\s_{i,k}|\s_{i,j}).
% \end{equation}
% Now, $H(\s_{i,j}) \geq \max\{H(\s_{i,j}|\s_{j,k}), H(\s_{i,j}|\s_{i,k})\}$. If $\x$ is sampled from a distribution $P_{\X}$, then we have that 
% \begin{equation}
%     H(\s_i) - H(\x_i) \geq \max\{B_1^{(i,j,k)},B_2^{(i,j,k)}\}
% \end{equation}
% where $B_1^{(i,j,k)}$ and $B_2^{(i,j,k)}$ are as defined above. 
% \end{proof}
% We now explain how to obtain a bound on $B_1^{(1,2,3)}$ and $B_2^{(1,2,3)}$. We first expand $B_1^{(1,2,3)}$ and $B_2^{(1,2,3)}$ using the following two lemmas. 

% \begin{definition}
%     For $l \in \cN$, the set of distributions
%     \begin{equation}
%         \cP_{\cS}^l(p) := \left\{Q_{\X} \in \cP_{\cS} | Q_{\x_l} = p\right\}
%     \end{equation}
%     where $Q_{\x_l} = \sum_{\cN \setminus \{l\}} Q_{}$
% \end{definition}

% \begin{lemma}
%     For a given scheme $\scheme$ which generates shares according to the distribution $P_{\s|\x}$ such that $\x$ is coming from a space $\cS$, 
%     \begin{equation}
%         \max_{P_{\X} \in \cP_{\cS}} B_1^{(i,j,k)} \geq \max_{P_{\X} \in \cP_{\cS}} \left\{\max_{} \right\}
%     \end{equation}
% \end{lemma}

% \begin{theorem}
% \end{theorem}


\section{Developing the Lower Bound}
\label{bounddevelop}
We now develop a lower bound on the randomness complexity. We first give a lemma which gives the bound in terms of conditional entropies.

\begin{lemma}
\label{boundlemma1}
For a secret sharing scheme $\scheme$ generating shares according to the distribution $P_{\Shares|\Secrets}$ such that $\Secrets$ is sampled from the space $\cS$,
\begin{equation}
    \rc \geq H(\Sa) - H(\Xa)
\end{equation}
\end{lemma}
% \rc \geq \max_{P_{\X}\in\cP_{\cS}} \{H(\Sab|\Sca) + H(\Sca|\Sab) - H(\Xa)\}
\begin{proof}
% Consider the distribution $P_{\s,R|\x}(w,r|x)=P_{R|\x}(r|x)P_{\s|\x,R}(w|x,r)=P_{R}(r)\mathbb{1}_{w=\encoder(x,r)}$, $w \in \salp$, $r \in \cR$ and $x \in \cS$. This gives
The joint distribution over $\Secrets, \Shares$ and $R$ gives that 
$$H(\Shares,R|\Secrets) = H(R|\Secrets)+H(\Shares|R,\Secrets) = H(R)$$
\begin{align}
\rho &= \log|\cR| \geq H(R) \geq H(\Shares|\Secrets)\\
&= H(\Sab, \Sbc, \Sca|\Xa,\Xb,\Xc)
\end{align}
% where $\cP_{\cS} := \{P_{\X}|\text{ Supp}(P_\x)\subseteq \cS \}$.
% We denote $\x = (\Xa,\Xb,\Xc)$ and $x = (\xa,\xb,\xc)$.
    % \begin{align*}
    %     % \rc &\geq H(\s|\x)\\
    %     &= 
    %     % &\geq \max_{P_{\X} \in \cP(\cS)}
    %     % &\geq \max_{P_{\X} \in \pins} \{H(\Sab|\Xa)+H(\Sca|\Xa)\}
    % \end{align*}
    Dropping the entropy due to $\Sbc$, 
    \begin{align}
        \label{exp1}
        \rc &\geq H(\Sa|\X)\\
        &\stackrel{(a)}{=} H(\Sa|\Xa)\\
        \label{exp2}
        &\geq H(\Sa) - H(\Xa)
    \end{align}
    where (a) is because of privacy condition.
\end{proof}

As we further explain in lemma \ref{generallemma}, we further bound the term $H(\Sab,\Sca)$ with $H(\Sab|\Sca) + H(\Sca|\Sab)$ and so on. These quantities have $P_{\X}$ as the input distribution. Now, the privacy criteria allows us to work with a different input distribution for both $H(\Sab|\Sca)$ and $H(\Sca|\Sab)$ (where both these input distributions are potentially different from $P_{\X}$). Working with different input distribution potentially gives us a better bound on the terms $H(\Sab|\Sca)$ and $H(\Sca|\Sab)$ individually which gets us a better lower bound. We explore this idea in the following lemma $\ref{distswitch}$.

% As we further explain in the lemma \ref{generallemma}, we further expand the term $H(\Sab,\Sca)$ as $H(\Sab|\Sca)+H(\Sca)$ and bound these terms individually. Before that, we first introduce lemma \ref{distswitch} which will let us choose the distributions on these expanded parts individually. For instance, note that the term $(\Sab|\Sca)$ is independent of $(\Xb,\Xc)$ conditional on $\Xa$ due to privacy. This enables us to use a different distribution to work with (say $P'_{\X} \in \pins$) as we bound the term $H(\Sab|\Sca)$ than what we had initially (which is $P_\x$). This is explained in the following lemma.

% Expanding $H(\Sa)$ as $H(\Sab)+H(\Sca|\Sab)$, we have
%     \begin{equation}
%     \label{exp3}
%         \rc \geq \max_{P_{\X} \in \pins} \{H(\Sab) + H(\Sca|\Sab) - H(\Xa)\}   
%     \end{equation}
%     Further, bounding $H(\Sab)$ with $H(\Sab|\Sca)$, we have,
%     \begin{equation}
%     \label{exp4}
%         \rc \geq \max_{P_{\X} \in \pins} \{H(\Sab|\Sca) + H(\Sca|\Sab) - H(\Xa)\}
%     \end{equation}

\begin{lemma}
\label{distswitch}
    Consider the set  $\pins^i(P):=\left\{Q_{\Xa,\Xb,\Xc} \in \pins| Q_{\X_{j}}=P\right\}$ where $Q_{\X_{j}}$ is the marginal of $Q_{\Xa,\Xb,\Xc}$ over $\X_j$ such that $j\in [3]$. Then we have that 
    \begin{equation}
        H(\Sab,\Sca) = \max_{P_{\X'}\in \pinsa\left(P_{\Xa}\right)} H(\Sab',\Sca')
    \end{equation}
    where 
    \begin{multline}
        P_{\Sab',\Sca'}(\sab,\sca)\\ := \sum_{x \in \cS}P_{\X'}(\x) P_{\Sab,\Sca|_\X}(\sab,\sca|\x)
    \end{multline}
\end{lemma}

\begin{proof}
    For $P_{\X'} \in \pinsa\left(P_{\Xa}\right)$, $P_{\Xa'} = P_{\Xa}$. Using this, we have 
    \begin{multline}
        P_{\Sab',\Sca'}(\sab,\sca)\\ = \sum_{\x\in\cS} P_{\Xa}(\xa)P'_{\Xb,\Xc|\Xa}(\xb,\xc|\xa) P_{\Sab,\Sca|\X}(\sab,\sca|x)
    \end{multline}
    From privacy condition, we have that
    \begin{multline}
        P_{\Sab,\Sca|\Xa,\Xb,\Xc}(\sab,\sca|\xa,\xb,\xc) \\= P_{\Sab,\Sca|\Xa}(\sab,\sca|\xa).
    \end{multline}
    Using this, we have that for $P'_{\Xa} \in \pins^1(P_{\Xa})$, $P_{\Sab',\Sca'} \equiv P_{\Sab,\Sca}$.
    So, corresponding entropies will be equal which gives the required result. 
\end{proof}

We now expand the term $H(\Sa)$ and using lemma \ref{distswitch}, we write two bounds on the randomness complexity. We will use the definitions written in lemma \ref{distswitch} for writing the further bounds as well. 

\begin{lemma}
\label{generallemma}
For a secret sharing scheme $\scheme$ which distributes shares according to distribution $P_{\Shares|\Secrets}$ and $\Secrets$ is sampled from a set $\cS$, the randomness complexity can be bounded as
    \begin{multline}
    \label{fullbound1}
        \rc \geq \max_{P_{\X}\in\pins} \left\{\max_{P_{\X'} \in \pinsa(P_{\Xa})}\{H(\Xa',\Xb'|\Xc')+RI(\Xa';\Xc')\} \right. \\+  \left. \max_{P_{\X''} \in \pins^1(P_{\Xa})} \{H(\Xc'',\Xa''|\Xb'')+RI(\Xa'';\Xb'')\}-H(\Xa) \right\} 
    \end{multline}
    and 
    \begin{multline}
    \label{fullbound2}
        \rc \geq \max_{P_{\X}\in\pins} \left\{\max_{P_{\X'} \in \pinsb(P_{\Xb})}\{H(\Xa',\Xb'|\Xc')+RI(\Xb';\Xc')\} \right. \\+  \left. \max_{P_{\X''} \in \pins^1(P_{\Xa})} \{H(\Xc'',\Xa''|\Xb'')+RI(\Xa'';\Xb'')\}-H(\Xa) \right\}.
    \end{multline}
\end{lemma}

\begin{proof}
    We start from the expansion obtained in lemma \ref{boundlemma1}. Suppose we have a distribution $P_{\X}$ on the secrets. Then schemes alongwith the secrets imply the following
    \begin{align}
        \rc &\geq H(\Sa) - H(\Xa)\\
        \label{exp3}
        &= H(\Sab)+H(\Sca|\Sab) - H(\Xa)\\
        \label{exp4}
        & \geq H(\Sab|\Sca)+H(\Sca|\Sab)-H(\Xa)
    \end{align}
    Note that the input distribution for both $H(\Sab|\Sca)$ and $H(\Sca|\Sab)$ is $P_{\X}$. We can switch the input distribution of $H(\Sab|\Sca)$ to $P_{\X'} \in \pinsa(P_{\Xa})$ and the input distribution of $H(\Sca|\Sab)$ to $P_{\X''}\in\pinsa(P_{\Xa})$ according to lemma \ref{distswitch} and write the bound as
    \begin{multline}
        \rc \geq \max_{P_{\X'} \in\pinsa(P_{\Xa})} H(\Sab'|\Sca')\\ + \max_{P_{\X''} \in \pinsa(P_{\Xa})} H(\Sca''|\Sab'') - H(\Xa) 
    \end{multline}
    Using lemma \ref{naivelemma} and \ref{rilemma}, we can bound
    \begin{align*}
        H(\Sab'|\Sca') &= H(\Sab'|\Sca',\Sbc') + I(\Sab';\Sbc'|\Sca')\\
        & \geq H(\Xa',\Xb'|\Xc') + RI(\Xa';\Xc')
    \end{align*} and similarly
    \begin{align*}
        H(\Sca''|\Sab'') \geq H(\Xc'',\Xa''|\Xb'') + RI(\Xa'';\Xb'').
    \end{align*}
    This gives the bound in (\ref{fullbound1}). 
    Now, $H(\Sab)$ in (\ref{exp3}) can also be bounded as $H(\Sab) \geq H(\Sab|\Sbc)$ to get another bound 
    \begin{equation}
        \rc \geq H(\Sab|\Sbc) + H(\Sca|\Sab) - H(\Xa)
    \end{equation}
    If the distribution input to $H(\Sab|\Sbc)$ can be changed to some $P_{\X'}\in\pinsb(P_{\Xb})$ and the distribution for $H(\Sca|\Sab)$ can be switched in the same way as before, using lemma \ref{boundlemma1} and lemma \ref{rilemma} we can bound
    \begin{align*}
        H(\Sab'|\Sbc') &= H(\Sab'|\Sca',\Sbc') + I(\Sab';\Sca'|\Sbc')\\
        & \geq H(\Xa',\Xb'|\Xc') + RI(\Xb';\Xc')
    \end{align*}
    which gives the bound in (\ref{fullbound2}).
\end{proof} 

% \section{Examples}
% In this section, we give the procedure of obtaining the lower bounds on two classes of supports. Before going to the examples, we give a claim which computes the residual information.\\
% \textbf{Computation of Residual Information:} From definition (\ref{ridef}), we have that residual information between $X$ and $Y$ is the equal to the conditional mutual information $I(X;Y|Q^*)$ where $Q^*$ is the common random variable. Based on the computation of the common random variable, we give the following claim which computes the residual information:

% \begin{claim}
% \label{claim:RI=I}
%     For any two binary random variables $\Xa$ and $\Xa$ jointly distributed as $P_{\Xa,\Xb}$, the residual information $RI(\Xa;\Xb)=I(\Xa;\Xb)$ whenever 
% \end{claim}
% \begin{proof}
%     The characteristic bipartite graph between $\X_i$ and $\X_j$ will have four vertices, two vertices due to $\X_i$ on one of the sides and two vertices due to $\X_j$ on the opposite side. The vertices correspond to the characters $0$ and $1$ for both $\X_i$ and $\X_j$. It is easy to see that if $\cS$ is empty or if it has only element in it, then $RI(\X_i;\X_j)$=0. In other cases, the characteristic bipartite graph can either have one connected component or two connected components because $\cS \subseteq \{0,1\}^3$. When there is only a single connected component in the characteristic graph, then the common random variable is deterministic. Under this case, we have $RI(\X_i;\X_j)=I(\X_i;\X_j|Q^*)=I(\X_i;\X_j)$. When there are two connected components, the edges are either $\{(0,0), (1,1)\}$ or $\{(0,1), (1,0)\}$. Since, in this case, conditional on the connected component, the entropy on $\X_i$, $H(\X_i|Q^*)=0$, $RI(\X_i;\X_j)=I(\X_i;\X_j|Q^*)=0$.
% \end{proof}


\section{Secret Sharing Schemes}


\section{CMSS Schemes for Secrets with Binary Alphabets}
Consider that the secrets are sampled from a support $\cS \subseteq \{0,1\}^3$. In this section, we give secret sharing schemes when the secrets are known to be sampled from $\cS$ for every possible $\cS \subseteq \{0,1\}^3$. We also show that all the schemes considered here are optimal in the following sense: the randomness complexity of the scheme defined for secrets sampled from a certain support $\cS$ is equal to the lower bounds obtained for the randomness complexity when the secrets are known to come from $\cS$. There are $2^{2^3}=256$ possible supports associated with a space of 3 binary bits. But as we show later in this section, due to symmetry of many of these supports, we only need to consider schemes and lower bounds for 22 of them. We list them in table \ref{table:schemes}. In subsection \ref{subsec:sharessubsection}, we give the secret sharing schemes and in subsection \ref{subsec:boundsubsection}, we use the tools from section \ref{sec:bounddevelop} to give lower bounds on randomness complexity. 
\todo[inline]{reference for the table}


\subsection{Secret Sharing Schemes}
Here, we give the optimal schemes for secret sharing. Then, in the table[], we point to the scheme to be used in the corresponding support. Note that if a scheme is correct and secure for a certain support $\cS$, then it is correct and secure for all subsets of $\cS$.

\textbf{Scheme 1:} Consider ther support $\cS = \{0,1\}^3$, which is in fact, the full support. Since the correlations over this general support do not have any special properties, we would use a naive scheme which involves secret sharing every secret individually. The dealer would sample $\Ra, \Rb$ and $\Rc$ independently uniform Bernoulli. Secret $\Xa$ would be secret shared as $\Xa \oplus \Ra$ and $\Ra$ on different edges connecting to $\pa$. If we repeat the process for all the parties, the shares we get are the following:\\
$\Sab = (\Xa \oplus \Ra, \Rb)$, $\Sbc = (\Xb \oplus \Rb, \Rc)$ and $\Sca = (\Xc \oplus \Rc, \Ra)$. The correctness of this scheme is trivially easy to confirm. To see the privacy against $\pa$, note that $\pa$ receives $\Sab = (\Xa \oplus \Ra, \Rb)$ and $\Sbc = (\Xc \oplus \Rc, \Ra)$. Since $\Rc$ is uniformly independent of $\Ra$ and $\Rb$, $\Xc \oplus \Rc$ is indpendently uniformly random which hides $\Xc$ and $\Xb$ is not shared with $\pa$, $\pa$ learns nothing about $\Xa$ and $\Xc$ conditional on $\Xa$. Privacy can be argued against $\pc$and $\pb$ in a similar way. Note that this scheme is correct and private for secrets from any support $\cS \subseteq \{0,1\}^3$. The randomenss complexity of this scheme is 3 bits.

\textbf{Scheme 2:} Consider the support $\cS = \{(0,0,0), (0,1,1), (1,0,1), (1,1,0)\}$. Note that in this support, $\Xa=\Xb \oplus \Xc$, $\Xb=\Xc \oplus \Xa$ and $\Xc = \Xa \oplus \Xb$. The dealer samples one Bernoulli uniform coin $\Ra$ and generates the following shares: $\Sab = \Ra, \Sbc=\Xb \oplus \Ra$ and $\Sca=\Ra \oplus \Xa$. It is easy to see that every player can only recover its own secret and nothing more than that. Therefore the scheme is correct and secure.

\textbf{Scheme 3:} Consider the support $\cS = \{(0,0,0),(0,0,1),(1,1,0),(1,1,1)\}$. Note that in this support, $\Xa=\Xb$. This means that the dealer can assign the secret $\Sab=\Xa=\Xb$. For the secret $\Xc$, the dealer can sample a Bernoulli uniform variable $\Ra$ and can generate the shares $\Sbc=\Ra$ and $\Sca=\Ra \oplus \Xc$. $\pa$ and $\pb$ do not learn anything about $\Xc$ as $\Xc \oplus \Ra$ is also uniformly Bernoulli.

\textbf{Scheme 4:} Consider the support $\cS = \{(0,0,0),(0,0,1),(0,1,0),(0,1,1)\}$. Note that $\Xa=0$. The scheme is similar to scheme 1, the only difference being that $\Xa$ doesn't have to be secret shared. So, the shares are now $\Sab=\Rb$, $\Sbc=(\Xb \oplus \Rb, \Rc)$ and $\Sbc=(\Xc \oplus \Rc)$. The correctness and privacy can be argues similarly to scheme 1.

\textbf{Scheme 5:} Consider the support $\cS = \{(0,0,0),(0,0,1),(0,1,0),(1,0,0),(1,1,1)\}$. The scheme is given in algorithm \ref{alg:log6scheme}. Correctness of the scheme is easy to check case-by-case. To see that the scheme is private, note that when 

\begin{algorithm}
\caption{Secret Sharing Scheme for $\cS = \{(000),(001),(010),(100),(111)\}$}
    \begin{algorithmic}[1]    \label{alg:log6scheme}
        \REQUIRE:   Dealer recieves secrets $\Xa$, $\Xb$ and $\Xc$.
        \ENSURE:    Secerts are shared securely among the parties $\pa$, $\pb$ and $\pc$.
        \STATE      Dealer samples a random permutation $(\alpha, \beta, \gamma)$ of $(0,1,2)$. When $\Secrets=(000)$, $\Sab=\alpha, \Sbc=\beta$ and $\Sca=\gamma$. When $\Secrets=(111)$, $\Sab=\Sbc=\Sca=\alpha$. When $\X_i=1$ and $\X_j=\X_k=0$ where $(i,j,k)$ is a permutation over $[3]$, $\Share_i=\Share_{ij}=\Share_{ik}=\alpha$ and $\Share_{jk}=\beta$.
        \STATE      Parties decode their secrets $\X_i=1$ if both their shares are the same. Otherwise, they decode $\X_i=0$.
    \end{algorithmic}
\end{algorithm} 

We now point to the optimal scheme for every support $\cS \in \{0,1\}^3$ and give matching lower bound for the randomness complexity for every such support. Note that we only need to consider 22 of the supports due to symmetry. We call these supports 'representatives'. Let $\cS$ be a support. The set of supports which correspond to the representatives can be generated through the follwoing transformations.

\textbf{Negation:} $\cS' = \left\{ (\xa^{(l)} \oplus 1, \xb^{(l)}, \xc^{(l)})| \secrets^{(l)} \in \cS \right\}$ can be generated by negating $\xa$. Similar sets can be generated by negating $\xb$ and $\xc$. Note that the secret sharing scheme for such a support $\cS'$ is the same as the scheme for $\cS$ but with secrets negated appropriately. 

\textbf{Swapping coordinates:} $\cS' = \left\{(\x_i^{(l)}, \x_j^{(l)}, \x_k^{(l)}) | \secrets^{(l)} \in \cS \right\}$ can be obtained by swapping the coordinates according to any permutation $(i,j,k)$ on $\{1,2,3\}$. The secret sharing scheme for such a support $\cS'$ is the same as the scheme for $\cS$ but with secrets swapped appropriately.

These transformations are enlisted as figures in figure \ref{cubestable}. 
\todo[inline]{refer to the cube table ocrrectly in the appendix}.

\subsection{Lower Bounds on Randomness Complexity}
We now give two examples of computing the lower bound. For the rest of the representative functions, the lower bounds can be obtained by making the appropriate choices on expansions and distributions as given in the table \ref{table:schemes}. We only give the limiting optimizing distributions in the table. 

\textbf{Example 1:}
Consider a support $\cS = \{(000),(001),(010),(100)\}$. From theorem \ref{thm:RClowerbound}, we use the bound given in \ref{eq:LB2}. Let $\epsilon>0$. We choose the following distribution $P_{\Secrets}$:
\begin{align*}
    P_{\Secrets} (0,0,0) &= 1/3 (1-\epsilon) \quad P_{\Secrets} (0,0,1) = 1/3 (1-\epsilon)\\
    P_{\Secrets} (0,1,0) &= 1/3 (1-\epsilon) \quad P_{\Secrets} (1,0,0) = \epsilon
\end{align*}
This gives $H(\Xa)=H(\epsilon)$ and $P_{\Xb}(0)=(2+\epsilon)/3$.
Choose the following distribution $P_{\Secrets'}$:
\begin{align*}
    P_{\Secrets'} (0,0,0) &= P_{\Secrets'}(1,0,0) = (2+\epsilon)(1-\epsilon)/6\\
    P_{\Secrets'} (0,1,0) &= (1-\epsilon)/3 \quad P_{\Secrets'}(0,0,1) = (2+\epsilon)(\epsilon)/3
\end{align*}
To see that $RI(\Xb;\Xc)=I(\Xb;\Xc)$, note that the characteristic graph of the pair ($\Xb,\Xc)$ on the given support has a single connected component which makes the common random variable deterministic thus implying that the $CI_{GK}(\Xb;\Xc)=0$. Therefore, $H(\Xa',\Xb'|\Xc')+RI(\Xc';\Xb')=H(\Xb')+H(\Xa'|\Xb',\Xc')$
$$=H\left(\frac{1-\epsilon}{3}\right) + \left(\frac{(2+\epsilon)(1-\epsilon)}{3} \right)H\left( \frac{1}{2}\right) \text{.}$$
Choose the following distribution $P_{\Secrets''}$: 
\begin{align*}
    P_{\Secrets''}(0,0,0) &= P_{\Secrets}(0,0,1) = ((1-\epsilon)^2)/2\\
    P_{\Secrets''}(1,0,0) &= \epsilon \quad P_{\Secrets}(0,1,0) = \epsilon(1-\epsilon)
\end{align*}
To see that $RI(\Xa'';\Xb'')=I(\Xa'';\Xb'')$, note that the characteristic graph of the pair $(\Xa'',\Xb'')$ on the given support has a simgle connected component which makes the common random variable deterministic thus implying that the $CI_{GK}(\Xa'';\Xb'')=0$. Therefore, $H(\Xa'',\Xc''|\Xb'') + RI(\Xa'';\Xb'') = H(\Xa'')+H(\Xc''|\Xa'',\Xb'')$
$$=H(\epsilon) + (1-\epsilon)^2 H\left(\frac{1}{2} (1-\epsilon)^2\right) \text{.}$$
As $\epsilon \rightarrow 0, \rc^* \rightarrow \log_2 6$, where $\rc^*$ is the optimal $\rc$ obtained through the optimization. 

% \textbf{Example 2:}
% Consider the support $\cS = \{\}$. From theorem \ref{thm:RClowerbound}, we use the bound given in \ref{eq:LB1}. Let some $\epsilon>0$. We choose the follwoing distributions $P_{\Secrets}$:
% \begin{align*}
%     P_{\Secrets}(000)=P_{\Secrets}(001)=P_{\Secrets}(010)=P_{\Secrets}(011)=1/8\\
%     P_{\Secrets}(100)=P_{\Secrets}(110)=1/4-\epsilon/2\\
%     P_{\Secrets}(101)=\epsilon
% \end{align*}
% This gives $H(\Xa)=1$ and $P_{\Xa}(0)=P_{\Xb}(1)=1/2$.
% Choose $P_{\Secrets'}=P_{\Secrets}$ and $P_{\Secrets''}$ as follows:
% \begin{align*}
%     P_{\Secrets''}(000)=P_{\Secrets''}(001)=P_{\Secrets''}(010)=P_{\Secrets''}(011)=1/8\\
%     P_{\Secrets''}(100)=P_{\Secrets''}(101)=1/4-\epsilon/2\\
%     P_{\Secrets''}(110)=\epsilon
% \end{align*}
% This gives $H(\X)$

\begin{definition}
    For any party $\p_i, i \in [3]$ and any two secret vectors $\secrets=(\xa,\xb,\xc) \in \cS$ and $\secrets'=(\xa',\xb',\xc') \in \cS$ such that $\x_i=\x_i'$, the shares $\sharerv_i$ that $\p_i$ has access to must have the same support, i.e., 
    \begin{equation}
        \{\share_i \in \salp_i \colon P_{\sharerv_i|\Secrets}(\share_i|\secrets)>0\} = \{\share_i \in \salp_i \colon P_{\sharerv_i|\Secrets}(\share_i|\secrets')>0\}
    \end{equation}
\end{definition}
\begin{lemma}
    Any secret sharing scheme where the secret domain is $\cS = \{(0,0,0), (0,1,0), (1,0,0), (1,0,1)\}$ uses at least 3 bits of randomness. 
\end{lemma}
\begin{proof}
    Consider the encoder function $\encoder \colon \cS \times \cR \rightarrow \salpab \times \salpbc \times \salpca$. To show that $\rc = \log_2|\cR|$
\end{proof}

==> old_binary.tex <==
\section{3SS Schemes for Secrets with Binary Alphabets}a\label{sec:binary}
In this section, we characterize the randomness complexity of 3SS for the 255 distinct non-empty domains of secrets $\cS\subseteq\{0,1\}^3$.
As a first step, we drastically reduce the number of distinct supports for which randomness complexity needs to be characterized to 21.
For this, we observe that the randomness complexity of two supports $\cS,\cS'\subseteq\{0,1\}^3$ coincide if $\cS'$ can be obtained from $\cS$ using one of the following transformations:
In the sequel, for brevity, we denote $(x_1,x_2,x_3)\in\{0,1\}^3$ by simply $x_1x_2x_3$ wherever there is no room for confusion.
% such an abbreviation does not give way to confusion.
\begin{description}[style=unboxed,leftmargin=0cm]
    \item[Negation.] For some $i\in[3]$, $\cS'$ is obtained by negating coordinate $i$ of elements of $\cS$.
    e.g., for $i=1$, $x_1x_2x_3\in\cS'$ if and only if $\bar{x}_1x_2x_3\in\cS$, where $\bar{x}_1=1-x_1$.
    A scheme for $\cS$ can be used for $\cS'$ (and vice versa) if $\party{i}$ negates the output of the reconstruction function.
    %Thus, complexity is the same for both these supports.
    \item[Swapping coordinates.] For distinct $i,j\in[3]$, $\cS'$ is obtained by exchanging coordinates $i$ and $j$ of elements in $\cS$.
    e.g., for $(i,j)=(1,2)$, $x_1x_2x_3\in\cS'$ if and only if $x_2x_1x_3\in\cS$.
    A scheme for $\cS$ can be used for $\cS'$ (and vice versa) by exchanging the reconstruction functions of parties $\party{i}$ and $\party{j}$. 
    %Thus, complexity is the same for both these supports in this case as well.
\end{description}
Table~\ref{tab:cubestable} in Appendix~\ref{app:???} classifies all non-empty $\cS\subseteq\{0,1\}^3$ into 21 families such that any support in a family can be transformed to another from the same the family using a sequence of negations and swapping of coordinates. Thus all members of a family have the same randomness complexity.

%The randomness complexity of a representative member from each of the 21 families is presented in \cref{tab:my-table}.
%Here, we provide the information that will aid in comprehending the entries in the table.
%
%\subsection*{Understanding \cref{tab:my-table}}
%Each row of the table considers a representative domain of secrets from one of the aforementioned 22 families.
%For each row, we provide the randomness complexity of the domain, an RSS scheme achieving the optimal randomness complexity and a matching lower bound.
%In all our tables, we use a cube to visually represent each domain of secrets.
%The vertices of the cube are mapped to the Boolean hypercube $\{0,1\}^3$ as illustrated in the first row of the table.
%A secret domain $\cS\subseteq\{0,1\}$ is represented by a cube in which the vertex corresponding to each point $\secrets\in\cS$ is highlighted by a red ball.
%This provides a uniform representation of the secret domains; more importantly, equivalence of two domains in the same family as presented in \ref{cubestable} can be easily read off under this representation.
%
\input{table}
\subsection*{Randomness Optimal 3SS Schemes}
\Cref{tab:my-table} shows 3SS schemes which achieve optimal randomness complexity for each of the 21 aforementioned families.
%RSS schemes achieving optimal randomness complexity for each domain is described by defining the distribution from which the randomness is drawn and giving the map from the secrets and randomness to the shares.
\todo[inline]{Start cleaning up from here}
Several domains considered in the table share the same optimal RSS scheme, for example \textcolor{blue}{[list]}.
This is a consequence of the fact that an RSS scheme for $\cS\in\{0,1\}^3$ is also an RSS scheme for any $\cS'\subseteq\cS$ since the correctness and privacy for $\cS'$ is a subset of those for $\cS$.
We club such cases together to avoid repetition.
All presented schemes are easily verified to be perfectly correct, and hence, the reconstruction functions are implicit in the schemes.
We skip their description to avoid redundancy.

%%%%THIS IS NOT TRUE ANYMORE: In every RSS scheme in the table, each share is uniformly distributed in its domain irrespective of the value of the secret; this ensures that the privacy condition \eqref{eq:1-privacy} is met.
Furthermore, in most of the schemes \textcolor{blue}{[list]}, each secret $\secret{i}$ is shared by providing $R$ in $W_{ij}$ and $\secret{i}\oplus R$ in $W_{ki}$, where $R$ is a uniformly random bit independent of every other random variable.
This ensures that $\secret{i}$ can not be reconstructed only using $W_j$ or $W_k$; this ensures privacy against $\party{j}$ and $\party{k}$ is required in \eqref{eq:privacy-Pi}.

We now argue the privacy of two schemes that do not adhere to this pattern:

\noindent \textbf{Families (3), (7), (13)}. 
RSS scheme for $\cS$ using a uniformly random bit $R$ shares $\secrets$ as
\[ W_{ij}=R \oplus x_i\oplus x_j, \forall (i,j)\in\{(1,2),(2,3),(3,1)\}.\]
Note that $(W_{12},W_{31})$ is identically distributed as $(R',x_1\oplus R')$, when $R'$ is a uniform and independent bit.
Hence, it is identically distributed irrespective of all admissible values of $(x_2,x_3)$.
Thus, the scheme is perfectly correct and private against $P_1$.
Privacy against $P_2$ and $P_3$ can be argued similarly.

\noindent \textbf{Families (9), (11), (15)}.
The shares of each $\party{i}$ are the same random element if $x_i=1$, and distinct random elements otherwise.
This holds irrespective of the values of the other secrets.
Thus, the scheme is perfectly correct and private.

A formal proof of correctness and privacy of each RSS scheme employed in the table is provided in Appendix ??.

\subsection{Lower Bounds in \cref{tab:my-table}}
For all but \textcolor{blue}{5(?)} of the domains considered in \cref{tab:my-table}, tight lower bounds are obtained using \eqref{eq:LB2} in \cref{thm:RClowerbound} by appropriately choosing the distributions $P_{\Secrets},P_{\Secrets'}$ and $P_{\Secrets''}$.
We illustrate this using an example.
We will then describe how the information theoretic lower bounds in the table can be understood in an analogous manner.

\begin{example}
Let $\cS = \{000,001,010,100\}$.
We use the bound \eqref{eq:LB2} from theorem \ref{thm:RClowerbound}.
For $\epsilon>0$, define $P_{\Secrets}$ as
\begin{align*}
    P_{\Secrets} (000) &= (1-\epsilon)/3 \quad P_{\Secrets} (001) = (1-\epsilon)/3\\
    P_{\Secrets} (010) &= (1-\epsilon)/3 \quad P_{\Secrets} (100) = \epsilon
\end{align*}
With respect to $P_{\Secrets}$, $H(\Xa)=H(\epsilon)$ and $P_{\Xb}(0)=(2+\epsilon)/3$.
Next, define $P_{\Secrets'}$ and $P_{\Secrets''}$ belonging to family $\cP(P_{\Xa})$, i.e., $P_{\Secrets'},P_{\Secrets''}$ such that $P_{\Xa'}=P_{\Xa''}=P_{\Xa}$, as follows:
\begin{align*}
    P_{\Secrets'} (000) &= (2+\epsilon)(1-\epsilon)/6 \quad &&P_{\Secrets'} (010) = (1-\epsilon)/3\\
    P_{\Secrets'}(100) &= (2+\epsilon)(1-\epsilon)/6 \quad &&P_{\Secrets'}(001) = \epsilon(2+\epsilon)/3
\end{align*}
and
\begin{align*}
    P_{\Secrets''}(000) &= ((1-\epsilon)^2)/2 \quad &&P_{\Secrets}(001) = ((1-\epsilon)^2)/2\\
    P_{\Secrets''}(100) &= \epsilon \quad &&P_{\Secrets}(0,1,0) = \epsilon(1-\epsilon)
\end{align*}
With respect to $P_{\Secrets'}$, the characteristic graph of random variables ($\Xb',\Xc')$ is connected.
Hence, $CI_{GK}(\Xb';\Xc')=0$, and $RI(\Xb';\Xc')=I(\Xb';\Xc')$.
Furthermore, $RI(\Xa'';\Xb'')=I(\Xa'';\Xb'')$ with respect to $P_{\Secrets''}$ as well since the characteristic graph of ($\Xa'',\Xb'')$ is also connected.
Then,
\begin{align*}
    \rc
    &= H(\Xa',\Xb'|\Xc')+RI(\Xc';\Xb')\\
    &\hspace{2cm} + H(\Xa'',\Xc''|\Xb'')+RI(\Xa'';\Xb'')-H(\Xa)\\
    &=H(\Xa',\Xb'|\Xc')+H(\Xb')-H(\Xb'|\Xc')\\
    & + H(\Xa'',\Xc''|\Xb'')+H(\Xa'')-H(\Xa''|\Xb'') - H(\Xa)\\
    &=H(\Xb')+H(\Xa'|\Xb',\Xc')+H(\Xc''|\Xa'',\Xb'')
\end{align*}
Plugging in these values according to $P_{\Secrets'}$ and $P_{\Secrets''}$,
\begin{align*}
    \rc
    &= H\left((1-\epsilon)/3\right) + (2+\epsilon)(1-\epsilon)H(1/2)/3\\
    &\hspace{1cm} + H(\epsilon) + (1-\epsilon)^2 H\left((1-\epsilon)^2/2\right).
\end{align*}
As $\epsilon \rightarrow 0, \rc \rightarrow \log_2 6$. 
\end{example}

For each domain other than \textcolor{blue}{[list]}, tight lower bound is obtained using an argument similar to the one sketched above.
Hence, we provide the distributions $P_{\Secrets},P_{\Secrets'}$ and $P_{\Secrets''}$ in the table that would replace their respective values in the above argument.
Note that, when a distribution is not supported on the entire domain, we only describe the distribution in the limit as $\epsilon$ goes to $0$.
The $\epsilon$ perturbations of such a distribution is obtained by simply moving $\epsilon$ mass from each point in the support to each point in the domain that is not included in the support.
\textcolor{blue}{For example...}
Thus, following the same line of argument as above, the lower bound on $\rc$ is given by the following expression evaluated with respect to $P_{\Secrets},P_{\Secrets'}$ and $P_{\Secrets''}$ provided in the table:
\begin{align*}
    \rc =H(\Xb')+H(\Xa'|\Xb',\Xc')+H(\Xc''|\Xa'',\Xb'').
\end{align*}

For domains \textcolor{blue}{[list]}, the bounds in \cref{thm:RClowerbound} fall short of being tight.
Hence, in each of these cases, we prove the optimality of the schemes in the table for these domains using a combinatorial proof.
The proof uses the perfect correctness and a weak notion of privacy implied by the privacy of RSS.
Below, we provide a proof sketch highlighting all the techniques used in proving a tight lower bound for \textcolor{blue}{domain number}.
Formal combinatorial proofs for domains \textcolor{blue}{[list]} are provided in Appendix ??.

\begin{example}
Let $\cS=\{000,010,100,101\}$ and $\scheme=(P_R,\encoder)$ be an RSS for $\cS$ with reconstructions functions $(\decoder_1,\decoder_2,\decoder_3)$.
For any $\secrets\in\cS$,
with $P_{\Shares|\Secrets}(\shares|\secrets)$ as defined in \eqref{eq:dealer-distr},
let
\[ M_{\secrets}=\{\shares\text{ s.t. } P_{\Shares|\Secrets}(\shares|\secrets)>0\}. \]
We prove $\rc\ge 3$ by showing that $|M_{100}|\ge 8$.

\noindent Let $a_1\in\salpab,b_1\in\salpbc,c_1\in\salpca$ such that
\begin{align}
P_{\Shares|\Secrets}(a_1b_1c_1|000)>0.\label{eq:comb0}
\end{align}
There exist $b_2\neq b_1$ such that
\begin{align}
    P_{\Shares|\Secrets}(a_1b_2c_1|010)>0 \label{eq:comb1}
\end{align}
This is argued as follows:
By privacy against $\party{1}$ in \eqref{eq:privacy-Pi},
\[ P_{\Sa|\Secrets}(a_1c_1|001) =  P_{\Sa|\Secrets}(a_1c_1|000) > 0.\]
However, $P_{\Shares|\Secrets}(a_1b_1c_1|010)=0$ since, by correctness for $\party{3}$, $\decoder_3(b_1c_1)=0$.
Thus, $P_{\Shares|\Secrets}(a_1b_2c_1|001)>0$ for some $b_2\neq b_1$.
Following similar line of arguments, appealing to appropriate privacy and correctness conditions, we can show that there exist $a_1\neq a_2\neq a_3\neq a_1$ and $c_1\neq c_2\neq c_3\neq c_1$ such that
\begin{align}
    P_{\Shares|\Secrets}(a_2b_1c_1|010)>0 
    \quad P_{\Shares|\Secrets}(a_1b_1c_3|101)>0 \label{eq:comb2}\\
    P_{\Shares|\Secrets}(a_1b_1c_2|100)>0 
    \quad P_{\Shares|\Secrets}(a_3b_1c_1|100)>0 \label{eq:comb3}
\end{align}
By privacy against $\party{3}$ in \eqref{eq:privacy-Pi},
\begin{align}
P_{\Sc|\Secrets}(b_1c_2|000) =  P_{\Sc|\Secrets}(b_1c_2|100) > 0.\label{eq:comb4}
\end{align}
Hence, there exists $a_4$ such that $P_{\Shares|\Secrets}(a_4b_1c_2|000)>0$.
However, by correctness of $\party{2}$ and the first condition in \eqref{eq:comb2}, $\decoder_2(a_2b_1)=1$;
and by correctness of $\party{1}$ and  the first condition in \eqref{eq:comb3}, $\decoder_1(a_1c_2)=1$.
But, we require $\decoder_2(a_4b_1)=0$ and $\decoder_1(a_4c_2)=0$, to ensure correctness for $\party{2}$ and $\party{1}$, respectively.
Hence, $a_4\notin \{a_1,a_2\}$.
At this point, the analysis branches into two cases: one where $a_4=a_3$ and one where $a_4\notin\{a_1,a_2,a_3\}$.
In the complete proof, provided in Appendix ??, we show that in both these cases, size of $M_{100}$ is necessarily at least 8, as required.
The proof proceeds by repeatedly appealing to privacy conditions and correctness conditions of appropriate parties along the lines of the arguments presented above.

% Since $a_1$ and $a_2$ are distinct, this implies there exist $b_3,c_3$ such that 
% \begin{align}
%     P_{\Shares|\Secrets}(a_2b_3c_3|000)>0.\label{eq:comb4}
% \end{align}
% This implies there exist $b_4\neq b_3$ and $c_4\neq c_3$ such that
% \begin{align}
%     P_{\Shares|\Secrets}(a_2b_4c_3|001)&>0, \label{eq:comb5}\\
%     P_{\Shares|\Secrets}(a_2b_3c_4|001)&>0,\label{eq:comb6}.
% \end{align}
% This can be shown using the same line of argument used to show, respectively, \eqref{eq:comb2} and \eqref{eq:comb3} starting with \eqref{eq:comb1}.
% Since $a_1\neq a_2,b_1\neq b_2,c_1\neq c_2,b_3\neq b_4$ and $c_3\neq c_4$, \eqref{eq:comb1}, \eqref{eq:comb2},\eqref{eq:comb5}, and \eqref{eq:comb6} imply that
% \[ |M_{001}| \ge |\{a_1b_2c_1,a_1b_1c_2,a_2b_3c_4,a_2b_4c_3\}| = 4.\]
% Thus, $\rc\ge 4$.
\end{example}


==> oldtable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\iffalse
\newcommand{\Depth}{0.5}
\newcommand{\Height}{0.5}
\newcommand{\Width}{0.5}

% #1 is scale, defaults to 1
\newcommand \drawcubea[1][1]%
{
    \coordinate (O) at (0,0,0);
    \coordinate (C) at (0,\Height*#1,0);
    \coordinate (G) at (0,\Height*#1,\Depth*#1);
    \coordinate (D) at (0,0,\Depth*#1);
    \coordinate (A) at (\Width*#1,0,0);
    \coordinate (B) at (\Width*#1,\Height*#1,0);
    \coordinate (F) at (\Width*#1,\Height*#1,\Depth*#1);
    \coordinate (E) at (\Width*#1,0,\Depth*#1);
    
    \draw (O) -- (A) -- (E) -- (D) -- cycle;% Bottom Face
    \draw (C) -- (B) -- (F) -- (G) -- cycle;% Top Face
    \draw (O) -- (C);
    \draw (A) -- (B);
    \draw (E) -- (F);
    \draw (D) -- (G);
}


\newcommand \drawballa[1]
{
    \shade[ ball color = red, opacity = 1.0] (#1) circle (0.1cm);
}

\newcommand{\drawFamilyOne}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyTwo}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D}}
            {
                \drawballa{\ballcoord} 
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyThree}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{G}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyFour}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{F}}
            {
                \drawballa{\ballcoord}
                
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyFive}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{A},{D}}
            {
                \drawballa{\ballcoord}
                
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilySix}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{B}}
            {
                \drawballa{\ballcoord}
                
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilySeven}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{G},{E}}
            {
                \drawballa{\ballcoord}
                
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyEight}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{A},{D},{E}}
            {
                \drawballa{\ballcoord}
                
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyNine}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{A}}
            {
                \drawballa{\ballcoord}
                
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyTen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{E}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyEleven}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{F}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyTwelve}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{B},{F}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyThirteen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{G},{E},{B}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyFourteen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{A},{B}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyFifteen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{A},{F}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilySixteen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{E},{B}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilySeventeen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{A},{B},{G}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyEighteen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{G},{E},{B}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyNineteen}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{E},{B},{F}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyTwenty}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{G},{A},{E},{B}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}

\newcommand{\drawFamilyTwentyOne}
{
    \begin{tabular}{c}
        \begin{tikzpicture}
            \drawcubea
            \shade[ball color=white, opacity=0.0] (C) circle(0.15cm);
            \foreach \ballcoord in {{O},{D},{C},{G},{A},{E},{B},{F}}
            {
                \drawballa{\ballcoord}
            }
        \end{tikzpicture}
    \end{tabular}
}


\begin{table*}[]
    \begin{tabular}{|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|@{ }c@{ }|}
    \hline
    Family & \begin{tabular}[c]{p{4cm}c}
        Representative $\cS \subseteq \{0,1\}^3$\ shown as a subset of nodes in a cube that is labeled as here:& 
        \begin{tikzpicture}[baseline=10]
            \drawcubea[1.2]
            \node [above right,scale=0.6] at (O) {$000$};
            \node [above right,scale=0.6] at (A) {$100$};
            \node [right,scale=0.6] at (E) {$101$};
            \node [left,scale=0.6] at (D) {$001$};
            \node [left,scale=0.6] at (C) {$010$};
            \node [right,scale=0.6] at (B) {$110$};
            \node [right,scale=0.6] at (F) {$111$};
            \node [left,scale=0.6] at (G) {$011$};
        \end{tikzpicture}
    \end{tabular} & A randomness-optimal 3SS scheme for \cS   & $\rho$ \\ \hline \hline
    1        & $\drawFamilyOne$                                                      & $\Sab=\Sbc=\Sca=0$                                                                                &   \\ \cline{1-3}
    2        & $\drawFamilyThree$                                                    & $\Sab=\Sca=0$, and $\Sbc=\xb=\xc$                                                                 & 0 \\ \cline{1-3}
    3        & $\drawFamilyFour$                                                     & $\Sab=\Sbc=\Sca=\xa=\xb=\xc$                                                                      &   \\ \hline
    4 - 6    & $\drawFamilyTwo$ $\drawFamilySix$ $\drawFamilyTwelve$                 & $R \sim $ Bern(1/2), $\Sab = \Xa =\xb$, $\Sbc = R$, $\Sca = R \oplus \xc$                         & 1 \\ \hline
    7 - 8    & $\drawFamilySeven$ $\drawFamilyThirteen$                              & $R \sim $ Bern(1/2), $\Sab = R$, $\Sbc = R \oplus \xb$, $\Sca = R \oplus \xa$                     & 1 \\ \hline
    9 - 10   & $\drawFamilyFive$ $\drawFamilyEight$                                  & $R_1, R_3 \sim$ Bern(1/2), $\Sca=(R_1,R_3)$, $\Sab = \xa \oplus R_1$,  $\Sbc = \xc \oplus R_3$    & 2 \\ \hline
    11 - 13  & $\drawFamilyNine$ $\drawFamilyFifteen$ $\drawFamilyEleven$            & \begin{tabular}[c]{@{}c@{}}$(\alpha, \beta, \gamma)$ be a uniform permutation of $(0,1,2)$;\\
                                                                                               $(\Sab,\Sbc,\Sca)   = \begin{cases} 
                                                                                                                        (\alpha,\beta,\gamma) &\text{ if } \secrets = 000 \\
                                                                                                                        (\alpha,\alpha,\alpha) &\text{ if } \secrets = 111 \\
                                                                                                                        (\alpha,\beta,\alpha) &\text{ if } \secrets =  100\\
                                                                                                                        (\alpha,\alpha,\beta) &\text{ if } \secrets =  010\\
                                                                                                                        (\beta,\alpha,\alpha) &\text{ if } \secrets =  001 
                                                                                                                    \end{cases}$\end{tabular}                                             & $\log_2 6$ \\ \hline
    14 - 21  & \begin{tabular}[c]{@{}c@{}}$\drawFamilyTen$ $\drawFamilyFourteen$    $\drawFamilySeventeen$   $\drawFamilySixteen$ \\     
                                          $\drawFamilyEighteen$  $\drawFamilyNineteen$  $\drawFamilyTwenty$  $\drawFamilyTwentyOne$ \end{tabular} 
                                                                                     & \begin{tabular}[c]{@{}c@{}}$R_1,R_2,R_3 \sim$ Bern(1/2),\\
                                                                                        $\Sab = (\xa \oplus R_1 , R_2)$, $\Sbc = (\xa \oplus R_2, R_3)$, 
                                                                                        $\Sca = (\xa \oplus R_3, R_1)$ \end{tabular}                                                     & $3$ \\ \hline 
    \end{tabular}
    \caption{}
    \label{tab:my-table}
    \end{table*}
\fi


\begin{table*}[]
    \begin{tabular}{|c|c|c|c|}
    \hline
    \begin{tabular}[c]{@{}c@{}}Representative\\ member\\ image\end{tabular} & CMSS scheme for representative member                                                                                                                                                                                                                                                                                                                                    & Lower Bound Optimizing Distribution (equation \eqref{eq:LB2})                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}c@{}}Randomness\\ Complexity\end{tabular} \\ \hline
	1.$\drawFamilyOne$                                                      & $\Sab=\Sbc=\Sca=0$                                                                                                                                                                                                                                                                                                                                                       & \multirow{3}{*}{-}                                                                                                                                                                                                                                                                           & \multirow{3}{*}{0}                                              \\ \cline{1-2}
    2.$\drawFamilyThree$                                                    & $\Sab=\Sca=0$, and $\Sbc=\xb=\xc$                                                                                                                                                                                                                                                                                                                                        &                                                                                                                                                                                                                                                                                              &                                                                 \\ \cline{1-2}
    3.$\drawFamilyFour$                                                     & $\Sab=\Sbc=\Sca=\xa=\xb=\xc$                                                                                                                                                                                                                                                                                                                                             &                                                                                                                                                                                                                                                                                              &                                                                 \\ \hline
    4.$\drawFamilyTwo$                                                      & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Sample $R \sim $ Bern(1/2)\\ $\Sab = \Xa =\xb$\\ $\Sbc = R$\\ $\Sca = R \oplus \xc$\end{tabular}}                                                                                                                                                                                                                             & \multirow{3}{*}{$P_{\Secrets'}=P_{\Secrets''}=P_{\Secrets}: P_{\Xc}(0)=P_{\Xc}(1)=1/2$}                                                                                                                                                                                                      & \multirow{3}{*}{1}                                              \\ \cline{1-1}
    5.$\drawFamilySix$                                                      &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \cline{1-1}
    6.$\drawFamilyTwelve$                                                   &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \hline
    7.$\drawFamilySeven$                                                    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sample $R \sim $ Bern(1/2)\\ $\Sab = R$\\ $\Sbc = R \oplus \xb$\\ $\Sca = R \oplus \xa$\end{tabular}}                                                                                                                                                                                                                         & \multirow{2}{*}{$P_{\Secrets'}=P_{\Secrets''}=P_{\Secrets}: P_{\Xb}(0) = P_{\Xb}(1) =1/2$}                                                                                                                                                                                                   & \multirow{2}{*}{1}                                              \\ \cline{1-1}
    8.$\drawFamilyThirteen$                                                 &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \hline
    9.$\drawFamilyFive$                                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sample $R_2, R_3 \sim$ Bern(1/2)\\ $\Sca=(R_1,R_3)$\\ $\Sab = \xb \oplus R_2$, \\ $\Sbc = \xc \oplus R_3$\end{tabular}}                                                                                                                                                                                                       & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$P_{\Secrets}=P_{\Secrets}: \Xa=\Xb=0, P_{\Xc}(0)=1/2 $\\ $P_{\Secrets'}: \Xc=\Xb=0, P_{\Xa}=1/2$\\ $P_{\Secrets''}: \Xa=\Xb=0, P_{\Xc}=1/2$\end{tabular}}                                                                                      & \multirow{2}{*}{2}                                              \\ \cline{1-1}
    10.$\drawFamilyEight$                                                   &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \hline
    11.$\drawFamilyNine$                                                    & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Sample a random permutation \\ $(\alpha, \beta, \gamma)$ of $(0,1,2)$\\ If $\secrets = 000, \Sab=\alpha$,\\  $\Sbc=\beta, \Sca=\gamma$\\ If $\secrets=111, \Sab=\Sbc=\Sca=\alpha$\\ If for some $i \in [3], \x_i = 1$ and \\ $\x_j=0$ for $j \neq i,$\\ $\Shares_{ij}=\Shares_{ik}=\alpha, \Shares_{jk}= \beta$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}$P_{\Secrets}: P_{\Secrets}(000)=1/3, P_{\Secrets}(001)=1/3, P_{\Secrets}(010)=1/3$\\ $P_{\Secrets'}: P_{\Secrets'}(000)=1/3, P_{\Secrets'}(010)=1/3, P_{\Secrets'}(100)=1/3$\\ $P_{\Secrets''}: P_{\Secrets''}(000)=P_{\Secrets''}(001)=1/2$\end{tabular}        & $\log_2 6$                                                      \\ \cline{1-1} \cline{3-4} 
    12.$\drawFamilyFifteen$                                                 &                                                                                                                                                                                                                                                                                                                                                                          & \begin{tabular}[c]{@{}c@{}}$P_{\Secrets}: P_{\Secrets}(000)=1/3, P_{\Secrets}(001)=1/3, P_{\Secrets}(010)=1/3$\\ $P_{\Secrets'}: P_{\Secrets'}(000)=1/3, P_{\Secrets'}(010)=1/3, P_{\Secrets'}(100)=1/3$\\ $P_{\Secrets''}: P_{\Secrets''}(000)=P_{\Secrets''}(001)=1/2$\end{tabular}        & $\log_2 6$                                                      \\ \cline{1-1} \cline{3-4} 
    13.$\drawFamilyEleven$                                                  &                                                                                                                                                                                                                                                                                                                                                                          & combinatorial lower bound                                                                                                                                                                                                                                                                    & $\log_2 6$                                                      \\ \hline
    14.$\drawFamilyTen$                                                     & \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Sample $R_1,R_2,R_3 \sim$ Bern(1/2)\\ $\Sab = (\xa \oplus R_1 , R_2)$\\ $\Sbc = (\xa \oplus R_2, R_3)$\\ $\Sca = (\xa \oplus R_3, R_1)$\end{tabular}}                                                                                                                                                                         & combinatorial lower bound                                                                                                                                                                                                                                                                          & \multirow{8}{*}{3}                                              \\ \cline{1-1} \cline{3-3}
    15.$\drawFamilyFourteen$                                                &                                                                                                                                                                                                                                                                                                                                                                          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$P_{\Secrets}: P_{\Secrets}(000)=P_{\Secrets}(010)=1/2$\\ $P_{\Secrets'}: P_{\Secrets'}(000)=P_{\Secrets'}(100)=P_{\Secrets'}(010)=P_{\Secrets'}(110)=1/4$\\ $P_{\Secrets''}(000)=P_{\Secrets''}(001)=1/2$\end{tabular}}                          &                                                                 \\ \cline{1-1}
    16.$\drawFamilySeventeen$                                               &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \cline{1-1} \cline{3-3}
    17.$\drawFamilySixteen$                                                 &                                                                                                                                                                                                                                                                                                                                                                          & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}$P_{\Secrets}: P_{\Secrets}(000)=1/2, P_{\Secrets}(010)=1/2$\\ $P_{\Secrets'}: P_{\Secrets'}(001)=P_{\Secrets'}(010)=P_{\Secrets'}(101)=P_{\Secrets'}(110)=1/4$\\ $P_{\Secrets''}:P_{\Secrets''}(000)=1/2, P_{\Secrets''}(001)=1/2$\end{tabular}} &                                                                 \\ \cline{1-1}
    18.$\drawFamilyEighteen$                                                &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \cline{1-1}
    19.$\drawFamilyNineteen$                                                &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \cline{1-1}
    20.$\drawFamilyTwenty$                                                  &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \cline{1-1}
    \multicolumn{1}{|l|}{21.$\drawFamilyTwentyOne$}                         &                                                                                                                                                                                                                                                                                                                                                                          &                                                                                                                                                                                                                                                                                              &                                                                 \\ \hline
    \end{tabular}
    \caption{Old table}
    \label{tab:old-table}
    \end{table*}


==> schemes.tex <==
\subsection{Secret Sharing Schemes}
In this section, we develop CMSS schemes that achieve optimal randomness complexity for all the instances considered in \cref{table:schemes}.
It turns out that the optimal randomness complexity of each of the 22 instances considered in \cref{table:schemes} is achieved by one among five distinct secret sharing schemes.
This roots from the fact that a CMSS scheme for $\cS\in\{0,1\}^3$ is also a CMSS scheme for any $\cS'\subseteq\cS$ since the conditions to be met for perfect correctness and privacy for $\cS'$ is contained in the same for $\cS$.

Going forward, we illustrate aforementioned 5 CMSS schemes using examples, and argue their correctness and privacy.
The reader can convince themself of the correctness and privacy of these scheme as used in \cref{table:schemes} in an analogous manner.

\noindent \textbf{Scheme 1.} Let $\cS=\{0,1\}^3$.
Consider the CMSS scheme that shares each party's secret using a pair of additive secret shares;
i.e., secret $x_i$ is distributed as $R,x_i\oplus R$, where $R$ is a uniformly random bit.
Hence, when $\Ra,\Rb,\Rc$ are uniform and independent bits, to share $\secrets\in\cS$, the scheme sets
\begin{align*}
\Sab = (x_1 \oplus \Ra, \Rb),\\
\Sbc = (x_2 \oplus \Rb, \Rc),\\
\Sca = (x_3 \oplus \Rc, \Ra),
\end{align*}
Each $P_i$ recovers $x_i$ from $\randomcoin{i}$ and $x_i\oplus\randomcoin{i}$, but does not learn $x_j,j\neq i$ since it receives either $\randomcoin{j}$ or $x_j\oplus\randomcoin{j}$ which are both independent of $x_j$.
Finally, every individual share is a pair of uniform and independent bits irrespective of the secret.
This ensures perfect correctness and privacy.
% Observe that this is a valid scheme for any $\cS\subseteq\{0,1\}^3$. 

\noindent\textbf{Scheme 2.} Let $\cS = \{\secrets:x_1=0\}$.
The scheme for $\cS$ is similar to scheme 1, with the difference that $x_1$ need not be secret shared.
Hence, when $\Rb,\Rc$ are uniform and independent bits, to share $\secrets\in\cS$, the scheme sets
\begin{align*}
\Sab = (x_2\oplus \Rb) \quad \Sbc = (\Rb,\Rc) \quad \Sca = (x_3 \oplus \Rc)
\end{align*}
The correctness and privacy can be argued like in scheme 1.

\noindent \textbf{Scheme 3.} Let $\cS = \{\secrets\in\{0,1\}^3:x_1\oplus x_2\oplus x_3=0\}$.
CMSS scheme for $\cS$ using a uniformly random bit $R$ shares $\secrets$ as
\[ W_{ij}=R \oplus x_i\oplus x_j, \forall (i,j)\in\{(1,2),(2,3),(3,1)\}.\]
$P_1$ decodes $W_{12}\oplus W_{31}=x_2\oplus x_3$, which coincides with $x_1$ by definition of $\cS$.
$(W_{12},W_{31})$ is identically distributed as $(R',x_1\oplus R')$, when $R'$ is a uniform and independent bit.
Hence, it is identically distributed irrespective of all admissible values of $(x_2,x_3)$.
Each individual share is an independent bit irrespective of the secret.
Thus, the scheme is perfectly correct and private against $P_1$.
Correctness and privacy against $P_2$ and $P_3$ can be argued similarly.

\noindent\textbf{Scheme 4.} Let $\cS = \{\secrets\in\{0,1\}^3:x_1=x_2\}$.
CMSS scheme for $\cS$ using two uniform and independent bits $R,R'$ shares $(x_1,x_2,x_3)$ as
\[ \Sab=x_1+R \quad \Sbc=(R,x_3+R') \quad \Sca=(R,R')\]
$P_1$ and $P_2$ can recover $x_1$ which coincides with $x_2$.
$P_3$ recovers $x_3$ from $R'$ and $x_3\oplus R'$.
This ensures correctness.
Perfect privacy of the scheme can be easily verified.

\textbf{Scheme 5:} Let $\cS = \{(000),(001),(010),(100),(111)\}$.
Suppose $(\alpha,\beta,\gamma)$ is a random permutation of $(0,1,2)$.
The scheme shares $(x_1,x_2,x_3)$ as follows:
\begin{enumerate}
    \item If $\secrets=(000)$, $\Sab=\alpha, \Sbc=\beta$ and $\Sca=\gamma$.
    \item If $\secrets=(111)$, $\Sab=\Sbc=\Sca=\alpha$. 
    \item If, for some $i\in[3]$, $x_i=1$ and $x_j=0$ for $j\neq i$, $\Share_{ij}=\Share_{ik}=\alpha$ and $\Share_{jk}=\beta$.
\end{enumerate}
Each $P_i$ decodes $x_i=1$ if both their shares are the same, and $x_i=0$ otherwise.
Each share is individually a random element of $\{0,1,2\}$ irrespective of $\secrets$.
Furthermore, the shares of $P_i$ are the same random element if $x_i=1$, and distinct random elements otherwise.
This holds irrespective of the values of the other secrets.
Thus, the scheme is perfectly correct and private.

